Jet-Images: Computer Vision Inspired Techniques for Jet Tagging

We introduce a novel approach to jet tagging and classification through the use of techniques inspired by computer vision. Drawing parallels to the problem of facial recognition in images, we define a jet-image using calorimeter towers as the elements of the image and establish jet-image preprocessing methods. For the jet-image processing step, we develop a discriminant for classifying the jet-images derived using Fisher discriminant analysis. The effectiveness of the technique is shown within the context of identifying boosted hadronic W boson decays with respect to a background of quark- and gluon- initiated jets. Using Monte Carlo simulation, we demonstrate that the performance of this technique introduces additional discriminating power over other substructure approaches, and gives significant insight into the internal structure of jets.

==> Makefile <==
#All flows from here, your document should match this basename
BASENAME := JetImages

#Location of the programs
LATEX  := pdflatex -interaction=nonstopmode
BIBTEX := bibtex
SECTIONS := $(shell find ./ -name 'sec-*.tex')

#pattern which triggers a re-run of pdflatex
RERUN    := "(There were undefined references|Rerun to get (cross-references|the bars) right|Citation\(s\) may have changed.|Rerun to get outlines right)"
RERUNBIB := "No file.*\.bbl|Citation.*undefined"

ifneq ($(BIBTEX), )
	BIBFILES = JetImages.bib
endif


MARKERS="--------------------"

$(BASENAME).pdf: $(BASENAME).tex $(BIBFILES) $(SECTIONS) $(wildcard images/*)
	@echo "\n\n$(MARKERS) PDF $(MARKERS)\n\n"
	if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi
	$(LATEX) $(BASENAME).tex ; true
	@egrep $(RERUNBIB) $(<:%.tex=%.log) && (echo "\n\n$(MARKERS) Run bibtex to get citations right $(MARKERS)\n\n" ; $(BIBTEX) $(BASENAME))   ; true
	@egrep $(RERUN) $(<:%.tex=%.log)    && (echo "\n\n$(MARKERS) Rerun to get references right $(MARKERS)\n\n"     ; $(LATEX) $(BASENAME).tex); true
	@egrep $(RERUN) $(<:%.tex=%.log)    && (echo "\n\n$(MARKERS) Rerun again to get references right $(MARKERS)\n\n"     ; $(LATEX) $(BASENAME).tex); true

clean:
	rm $(BASENAME).pdf $(BASENAME).log $(BASENAME).toc.bak *.aux *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind 


